Analysis of Gender Inequality In Face Recognition Accuracy

We present a comprehensive analysis of how and why face recognition accuracy differs between men and women. We show that accuracy is lower for women due to the combination of (1) the impostor distribution for women having a skew toward higher similarity scores, and (2) the genuine distribution for women having a skew toward lower similarity scores. We show that this phenomenon of the impostor and genuine distributions for women shifting closer towards each other is general across datasets of African-American, Caucasian, and Asian faces. We show that the distribution of facial expressions may differ between male/female, but that the accuracy difference persists for image subsets rated confidently as neutral expression. The accuracy difference also persists for image subsets rated as close to zero pitch angle. Even when removing images with forehead partially occluded by hair/hat, the same impostor/genuine accuracy difference persists. We show that the female genuine distribution improves when only female images without facial cosmetics are used, but that the female impostor distribution also degrades at the same time. Lastly, we show that the accuracy difference persists even if a state-of-the-art deep learning method is trained from scratch using training data explicitly balanced between male and female images and subjects.

==> figures/fmr_fnmr_males_females_makeup.tex <==
\begin{figure*}[t]
  \begin{subfigure}[b]{1\linewidth}
      \begin{subfigure}[b]{0.32\linewidth}
          \begin{subfigure}[b]{1\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/morph/fmr_fnmr_MORPH_V2_C_makeup.png}
          \end{subfigure}
          \caption{MORPH Caucasian}
          \vspace{-0.5em}
      \end{subfigure}
      \hfill %%
      \begin{subfigure}[b]{0.32\linewidth}
          \begin{subfigure}[b]{1\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/nd/fmr_fnmr_ND_Genders_V3_C_makeup.png}
          \end{subfigure}
          \caption{Notre Dame}
          \vspace{-0.5em}
      \end{subfigure}
      \hfill %%
      \begin{subfigure}[b]{0.32\linewidth}
          \begin{subfigure}[b]{1\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{images/afd/fmr_fnmr_arcface_gender_AFD_makeup.png}
          \end{subfigure}
          \caption{AFD}
          \vspace{-0.5em}
      \end{subfigure}
  \end{subfigure}
  \caption{Male, female and female without makeup false match rate and false non-match rate.}
  \label{fig:fmr_fnmr_makeup}
  \vspace{-1em}
\end{figure*}

==> figures/skin_only_examples.tex <==
\begin{figure}[t]
  \begin{subfigure}[b]{1\linewidth}
      \begin{subfigure}[b]{1\linewidth}
          \begin{subfigure}[b]{.32\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{latex/images/morph_examples/skin_only/042028_0F51.JPG}
          \end{subfigure}
          \hfill %%
          \begin{subfigure}[b]{.32\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{latex/images/morph_examples/skin_only/053194_0F50.JPG}
          \end{subfigure}
          \hfill %%
          \begin{subfigure}[b]{.32\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{latex/images/nd_examples/skin_only/nd1S04446_Female_White_1984_2003-10-01_unavaliable_04446d231.JPG}
          \end{subfigure}
      \end{subfigure}
      \hfill %%
      \begin{subfigure}[b]{1\linewidth}
          \begin{subfigure}[b]{.32\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{latex/images/morph_examples/skin_only/048925_01M48.JPG}
          \end{subfigure}
          \hfill %%
          \begin{subfigure}[b]{.32\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{latex/images/morph_examples/skin_only/061692_3M41.JPG}
          \end{subfigure}
          \hfill %%
          \begin{subfigure}[b]{.32\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{latex/images/nd_examples/skin_only/nd1S04433_Male_White_1981_2003-01-23_04433d70_jpg_04433d70.JPG}
          \end{subfigure}
      \end{subfigure}
  \end{subfigure}
  \caption{Examples of images with hair and background removed on the MORPH African American (left), MORPH Caucasian (middle) and Notre Dame (right) datasets.}
  \label{fig:forehead_examples}
  \vspace{-1em}
\end{figure}

==> old_stuff/figures/fmr_fnmr.tex <==
\begin{figure*}
    \centering
        \subfigure{\includegraphics[width=0.3\linewidth]{latex/images/fmr_fnmr/58_gender_FMR.png}}
        \subfigure{\includegraphics[width=0.3\linewidth]{latex/images/fmr_fnmr/59_gender_FMR.png}}
        \subfigure{\includegraphics[width=0.3\linewidth]{latex/images/fmr_fnmr/FMR_gender_ResNet.png}}
        
        \subfigure{\includegraphics[width=0.3\linewidth]{latex/images/fmr_fnmr/58_gender_FNMR.png}}
        \subfigure{\includegraphics[width=0.3\linewidth]{latex/images/fmr_fnmr/59_gender_FNMR.png}}
        \subfigure{\includegraphics[width=0.3\linewidth]{latex/images/fmr_fnmr/FNMR_gender_ResNet.png}}
       % \subfigure{\includegraphics[width=0.3\linewidth]{latex/images/fmr_fnmr/FMR_Gender_Idemia.png}}
       % \subfigure{\includegraphics[width=0.3\linewidth]{latex/images/fmr_fnmr/FNMR_Gender_Idemia.png}}
    
    \caption{FMR and FNMR Comparison of Male / Female Accuracy for COTS-A, COT-B and ResNet Matchers. 
Annotated decision threshold points correspond to an FMR of 1-in-10,000 in both the FMR and FNMR figures.  The FNMR curves become noisy approaching a 1-in-1,000 FNMR due to the amount of data.
}
    \label{FMR FNMR Curves for all 4 matchers}
\end{figure*}


==> old_stuff/tables/dprime.tex <==
\begin{center}
\begin{tabular}{ |l||c|c|c|c|c|c| } 
 \hline
   \multirow{3}{*}{Dataset}    & \multicolumn{3}{|c|}{ArcFace}  & \multicolumn{3}{|c|}{ArcFace} \\
       & Male & Female & I+G & Male & Female & I+G \\ 
       &  d'   & F d'&  shift  &  d'   & F d'&  shift  \\ 
 \hline
 \hline
 Morph AA & 3.35 & 2.25 & yes & 3.35 & 2.25 & yes \\ 
 \hline
 Morph C  & 3.35 & 2.25 & yes & 3.35 & 2.25 & yes \\ 
 \hline
Morph & 3.35 & 2.25 & yes & 3.35 & 2.25 & yes \\ 
 \hline
ND    & 3.35 & 2.25 & yes & 3.35 & 2.25 & yes \\ 
 \hline
AFD    & 3.35 & 2.25 & yes  & 3.35 & 2.25 & yes \\  
\hline
\end{tabular}
\end{center}

==> old_stuff/tables/summary_table.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{ |l||c|c|c|c|c|c|c| } 
\hline
          & LBP  & COTS-A & COTS-B & COTS-C & FaceNet & VGGFace & ArcFace \\
\hline
\hline
Morph A-A &      &      &   &     &          &         &  \\
Male d'   &      &      &   &     &  3.35    &  3.35   &   3.35 \\
Female d' &      &      &   &     &  2.25    &  2.25   &   2.25 \\
I Shift   &      &      &   &     & Y        &   Y     &    Y \\
G shift   &      &      &   &     & Y        &   Y     &    Y \\
 \hline
Morph C   &      &      &   &     &          &         & \\
Male d'   &      &      &   &     &  3.35    &  3.35   &   3.35 \\
Female d' &      &      &   &     &  2.25    &  2.25   &   2.25 \\
I Shift   &      &      &   &     & Y        &   Y     &    Y \\
G shift   &      &      &   &     & Y        &   Y     &    Y \\
 \hline
ND        &      &      &   &     &          &         & \\
Male d'   &      &      &   &     &  3.35    &  3.35   &   3.35 \\
Female d' &      &      &   &     &  2.25    &  2.25   &   2.25 \\
I Shift   &      &      &   &     & Y        &   Y     &    Y \\
G shift   &      &      &   &     & Y        &   Y     &    Y \\
 \hline
AFD       &      &      &   &     &          &         & \\
Male d'   &      &      &   &     &  3.35    &  3.35   &   3.35 \\
Female d' &      &      &   &     &  2.25    &  2.25   &   2.25 \\
I Shift   &      &      &   &     & Y        &   Y     &    Y \\
G shift   &      &      &   &     & Y        &   Y     &    Y \\
 \hline
\end{tabular}
\end{center}
\end{table*}
